Astronomical Image Quality Prediction based on Environmental and Telescope Operating Conditions

Intelligent scheduling of the sequence of scientific exposures taken at ground-based astronomical observatories is massively challenging. Observing time is over-subscribed and atmospheric conditions are constantly changing. We propose to guide observatory scheduling using machine learning. Leveraging a 15-year archive of exposures, environmental, and operating conditions logged by the Canada-France-Hawaii Telescope, we construct a probabilistic data-driven model that accurately predicts image quality. We demonstrate that, by optimizing the opening and closing of twelve vents placed on the dome of the telescope, we can reduce dome-induced turbulence and improve telescope image quality by (0.05-0.2 arc-seconds). This translates to a reduction in exposure time (and hence cost) of $\sim 10-15\%$. Our study is the first step toward data-based optimization of the multi-million dollar operations of current and next-generation telescopes.

==> Old_Files/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}


==> Old_Files/data.tex <==
\section{Data} \label{sec:data}
%Describe the data\\
%- the CFHT, dome, sensors, instruments\\
%- archived data, pre-processing, post-processing

Almost two decades worth of Megaprime (the CFHT wide field optical imager) IQ measurements have been archived at CFHT. %and CADC, 
%which we use as targets in this work. Along  with accompanying observatory and environmental parameters, 
Prior to use in our neural network we performed significant pre-processing.  Pre-processing was neccessary due to features being spread across multiple data sets, the need for calibration,
%exposures contained both sidereal and non-sidereal observations, 
and data records contained missing data due to sensor failures.
We have made the cleaned data sources publically available at \tcr{[ link.]}
%data was collected at an uneven cadence. 
%Here we briefly describe our data sources, cleaning procedures, and undertaken engineering steps.

%Before using our data with our model, we first perform data cleaning and engineering. %The former refers to identification of removal of outliers and errant values, while the latter refers to both application of various statistical procedures to existing features, and their usage in the construction of new features using expert knowledge to make them more amenable for use by neural networks.While data cleaning is a necessary first step of any ML pipeline, feature engineering is an optional but often desirable step that increases the predictive capacity of models. In \S\ref{sec:rawData} we describe in detail the various subsets of our collated data set, and briefly introduce the instruments from which they were collected. We then expound on our data cleaning and feature engineering procedures in \S\ref{sec:data_cleaning} and \S\ref{sec:feature_engineering}, respectively.

%\subsection{Data sources}\label{sec:rawData}
%Our first step in data collection was to build a data archive that contains one data record per instrument exposure, for all five instruments used \yst{what are the five instruments?}. Throughout the rest of this article, we will refer to each exposure interchangeably as a sample and an observation.
Each input record
%/sample 
contains three distinct types of predictive variables. %\sg{(Sankalp: we could perhaps put in the median time of MegaCam exposures? and a plot with histogram of exposure times?)}.
The first type are dome operating parameters, which
%.  These \textbf{are typically fixed} for the duration of the exposure and 
include 
%variables such as
the telescope altitude and azimuth 
%(in degrees) 
during the period of image forming,  configurations of the twelve dome vents (open or closed), and the windscreen setting (degrees open). These are the actionable parameters that we attempt to optimize
%to reduce the dome-induced turbulence. 
The second type consists of statistical information on environmental conditions.
%over the period of the exposure. There are
%collected by the \textbf{xxx} sensors in and around telescope. 
%in total. 
%These environmental variables 
%Examples of the data collected 
These include the %median 
wind speed over the duration of the exposure, wind direction, barometric pressure, and various temperature sensors 
%sensors 
placed both inside and outside of the dome. Finally we have ancillary information of the telescope such as the dome ``pointing'', i.e., which astronomical object is being observed.  
%The final type is the MKAM instrument which came online in 2009.  MKAM is a smaller instrument housed separately from MegaCam \textbf{insert citation}, which provides profile FWHM estimates every 60 seconds.  In our dataset we provide the average MKAM IQ estimate over the duration of the MegaCam exposure. %\yst{just making sure I understand, we input also MKAM IQ to predict MegaCam IQ?}.
In total there are \tcr{\textbf{xxx}} predictive variables provided with each exposure.  The  total is \tcr{\textbf{xxx}} records, spanning observations made from \tcr{\textbf{month/year}} to \tcr{\textbf{month/year}}. %We used this dataset in \S\ref{sec:DL_SL} in our supervised results. \yst{Maybe a table summarizing the variables.}

%Our second step in data collection was to complement the initial archive with seeing data from other instruments. Since instruments are routinely swapped to meet differing science goals, no single instrument is uninterruptedly in operation at CFHT. These other instruments are online in period for which MegaCam was offline and include SPIRou, SITELLE, and WIRCam \seb{probably ESPaDOnS as well?}.  SPIRou is a near-infrared spectropolarimeter. SITELLE is a wide-field Fourier transform spectrograph. WIRCam is composed of four infrared detectors optimized for the J, H, and K spectral bands.  Respectively these instruments add \tcr{$150,000$, $85,000$ and $100,000$} records to the data archive.  \tcr{(SCD: I think the above may be old numbers)} Each of these instruments  produces an IQ measurement \seb{might be worth mentioning how those IQ measurements are performed - and when relatively to MCAM}.  And each data record here contains one such IQ measurement plus the same predictive variables on environmental conditions and operating parameters as for MegaCam.  This data set consists of \tcr{xxx} records, spanning observations made from \tcr{month/year} to \tcr{month/year}. As the IQ produced by these instruments is not the same as that produced by MegaCam, we use these latter data in \S\ref{sec:DL_SSL} in our semi-supervised results.  

%Our archive combines the measurements of all instruments in a single unified formatting.  When a measurement is not available, e.g., there is no MegaCam IQ data, or when a sensor has failed, we populate the missing field with ``NaN''.  \yst{Did we end up doing data inputation?} We also note that the cadence of the data varies both across instruments and for each instrument.  For example, MegaCam exposure length varies from around \tcr{xxx} seconds on the short end to \tcr{xxx} seconds on the long end.  \tcr{We describe these steps Figure ()() through (). }

The dome vents are of particular importance.
%particularly important to understand. 
They were installed in 2012 to allow for colder mountain air to `flush out' the heated air inside the dome, in an attempt to reduce the dome-induced turbulence. Unfortunately, in practice, the vent positions have barely been changed.
%\emph{dome seeing}--the portion of the IQ that can be attributed to turbulent air between the telescope mirror and the dome shutter \citep{wind_tunnel_test}. 
An important goal of this work is to discover relationships between opening and closing
%the ON/OFF positions 
of these vents, and the observed Megacam image quality 
%with a goal 
and to find optimal vent positions as a function of other features. 
%Since their installation, the vent positions have barely been changed--see Figure () comparing the different vent configurations as a function of time.

%\iffalse
%\begin{figure}
   % \centering
    %\includegraphics[width=\textwidth]{ventlocs.png}
    %\caption{Caption}
   % \label{fig:my_label}
%\end{figure}
%\fi

%\iffalse

\begin{enumerate}
%    \item The data records corresponding to the most recent 18 months of experiments are  proprietary.  As these data are not yet in the public domain we remove proprietary data including identifying information such as investigator name and program and target identity. \seb{some of the metadata is actually proprietary too - especially spirou}
    %%%%%%%%%%%%%%%%%%
  %  \item Next, we remove moving, non-sidereal, targets. The images of stars are ``smeared'' in such images.  The result is a highly eccentric reception field that translates to a poor estimate of IQ. These data records are therefore not appropriate for training. %As part of the configuration files the astronomers defined for their observation they specify whether the observation is sidereal or not, hence these data records are easy to remove from the training set.
%    \sg{Sankalp: Billy, HOW exactly are these identified?} \bm {when astronomers define the configuration for their observations, they can a specify non-sidereal or sidereal setup.  when i extract the data, i join to this table and filter the non-sidereal data.  It might be possible to use the eccentricity metric from processed data, but I've not personally performed that reduction or executed that exercise.}
    %%%%%%%%%%%%%%
    %\item Data records corresponding either to short exposures or unrealistic IQs 
    %are too small or excessively large
    %are also removed. In prior studies\tcr{(add citation -- can we also say *why* these were removed? Do we think the big end is non-sidereal?)} \sg{Sankalp: Billy put this in, I'll ask him to clarify} exposures of less than 30 seconds were removed; we do the same.
    %%%%%%%%%%%
    %\item %\tcr{(SCD: This sentence is in the draft but I don't see what it has to do with the 0.15" and 3.0" that follows: "The real time analysis of a Megacam acquisition produces an image quality (IQ) measurement reported specifically for the band/filter it was acquired under.")}
    %Megacam exposures associated with IQ measurement of less than 0.15" or greater than 3.0" are removed from the data set as these IQ numbers are deemed unrealistic.  \textbf{(SCD: can we say what "unrealistic" means -- a sensor failure?)} \textbf{these are conversational constraints, I dont have a citation, in the past work harvesting data for Rene and others, it was a constraint loosely placed on my work.  It has been 2.0,2.5, and 3.0 at various different points if i recall correctly.  I believe the discussed best skies over Mauna Kea yield seeing between .2 and .3". And seeing greater than 2.0" over Mauna Kea would be extremely gross for most science. (we are spoiled :)}\textbf{Sankalp: In that case, shouldn't the upper limit be a seeing of 2 and not 3 arcsecs?}
    %%%%%%%%%%%%%%%%
  %  \item Certain data records are made for calibration purposes.  These are non-science exposures necessary for post-acquisition analysis, e.g., imaging "biases", ``darks'' or ``flats''. \textbf{These targets don't yield good IQ estimates and so we exclude these records from the archive.}. 
    %Calibration data is removed from the data set. \tcr{(SCD: what is "calibration data"?)} \sg{Sankalp: Billy}  \bm {cals are non-science exposures but necessary to do the post-acquisition reductions and analysis.  cals can be "darks", "flats", etc. but typically these are non-IQ savvy data.}
    %\bm {for below the 3/5 5/3 math applies. its like .89 vs .83 and i'm curious how why they let that slip through.}
    %%%%%%%%%%%%%%
    %\item Since the IQ data varies with the band of observation, to make the IQ data compatible across data records, we scale all IQs to a common wavelength \textbf{how do you scale it?}. We choose this normalization wavelength to be $500$ nm \textbf{does this still make sense for the semi-supervised, since all IQ are "calibrated" to the Megacam IQ? Shouldn't another instrument or another filter be the same?}.  This is approximately in the middle of the MegaPrime range of operation.  We also remove a contribution to IQ from the instrument, ${\rm IQ}_{\rm Optics}$ which accounts for \textbf{xxx, yyy, zzz}.  The optics contribution is tabulated in Table \ref{table:opticsCorrection}. \textbf{dumb question: what is the Table about? How can we know the exact breakdown.. I am confused.} \textbf{(SCD: I don't know what this means.  Do you mean the table below -- I don't understand how those numbers map to these formulae.  Also, e.g., the first two entries are 0.49 and 0.20 and the total on the brackets is 0.35, what is the relationship here?)} \textbf{Sankalp: good catch--it's supposed to be 0.55, I fixed it. they still don't all sum to 0.89 by using the five-thirds forumula, and I don't honestly understand why. there might be clue to what's in the para right beneath Table 4 in \url{https://iopscience.iop.org/article/10.1086/605313/pdf?casa_token=lsAdKnzC_VYAAAAA:LIh4BUM21HLQZwOgOsatR2AKrKbo-PcI36ebBZvZJfod_ni-b1b-NHXu7_wCy72TS_cnCkhi-Y3kfsr542bj}, I'll have to read the paper because I can't really follow. Will get back to you. if you or Billy are able to go through it, please do.}
   % \textbf{i have a fit from Rene that I use to compute the Optics contribution in the table.  it is this value that i use in my reduction in the 5/3 3/5 math.  }
    %\textbf{this blurb is a historical note on the optics contributions to IQ, from an internal report not necessary to include, but you should read as an fyi: Image quality distributions and the effects of telescope optics Both the telescope optics and the atmosphere contribute to image blur. The best images occur when atmospheric seeing is minimum. If we assume that optics-related image blur is independent of telescope position and is reasonably constant over time, then we might reasonably assume the diameters of the best images to be a measure of the blur introduced by the telescope’s optics. We have therefore taken as the measure of optics induced blur, the X intercept of the extrapolated front edge of the image fwhm distributions for each MegaCam filter as depicted in Figure 9. In doing so, we realize this is a perhaps a pessimistic estimate of optical performance, and implies, rather optimistically, that there are rare moments in which atmospheric optical turbulence completely disappears. Nonetheless, these estimates of optical blur were arrived at in a consistent manner for each of the MegaCam filters, so we have used them in what follows. Figure 9 – the method used to establish image blur caused by telescope and camera optics For image blur contributed by telescope optics, we find:
%Filter optics fwhm effective wavelength (nm)
%u 0.54 arcsec* 374
%g 0.50 arcsec 487
%r 0.42 arcsec 625
%i 0.42 arcsec 770
%z 0.45 arcsec 890
 %- see Appendix IV for the u filter IQ histogram
%11
%\textbf{were the Halpha and CH&K filters also accounted?}
%Figure 10 – The histogram of MegaCam image fwhm for all filters \textbf{which measure of the FWHM was taken for the cuts? MCAM?} For each filters there was a tiny proportion of images with fwhm values better than the baseline optics contribution. These were removed from out data set since they lead to meaningless values in the next set of calculations, with the loss of 29 out of 10657 g images, 4 out of 12754 r images, 15 out of 7404 i images and 36 outof 5212 z images. However, this method of dealing with ‘outliers’ did not work well for the ‘u’ filter, where roughly 180 out of 2791 images had fwhm values smaller than the optics image quality derived by the method described above. We do not understand the source of this toe in the ‘u’ filter distribution and have therefore elected not to include ‘u’ filter data in our remaining work. The image fwhm distribution for each filter is provided in Appendix IV.}
   % \item A Finally, we note that IQ is affected by the amount of atmosphere through which the observation is made.  To normalize out this effect we compute a zenith angle correction where $z$ is the zenith angle in degrees. \textbf{I am confused, how do you get \textrm{IQ}_{\textrm{Dome}}??}
    
   % \begin{align*}
    %\textrm{IQ}_{\textrm{Atmosphere}} = \left(\textrm{IQ}_{\textrm{MegaCam}}^{5/3} - \textrm{IQ}_{\textrm{Optics}}^{5/3} - \textrm{IQ}_{\textrm{Dome}}^{5/3}\right)^{3/5}
    %\end{align*}%
    %After computing ${\rm IQ}_{\rm Atmosphere}$ we scaled the wavelength $\lambda$ (measured in nanometers) and the zenith angle $z$ (in degrees) as
    %\begin{align*}
       % \textrm{IQ}_{\textrm{Corrected}} = \textrm{IQ}_{\textrm{Atmosphere}} \times \left(\frac{\lambda}{500}\right)^{1/5} \times \left(\cos{z}\right)^{3/5}
    %\end{align*}
\end{enumerate}

%\subsection{Feature Engineering}
%\label{sec:feature_engineering}
%Creation of time features: Every observation/exposure has an associated time stamp, indicating the beginning of image acquisition. Using this `timestamp' feature, we derive several related features in order to capture any latent cyclical relationship between weather events and (): `hour of day', `day of week', `week of year', and `month of year'. Each of these four categorical features are further engineered into two new features, using \emph{cyclical encoding}: a `sinusoidal' component and a `co-sinusoidal component'. For example, for the `day of week' feature values--which can range from 0 to 6-- are converted to `day of week sin' and `day of week cos'--which take values from $\sin{\left(0\times180\degree/6\right)}$, to $\sin{\left(6\times180\degree/6\right)}$, and $\cos{\left(0\times180\degree/6\right)}$, to $\cos{\left(6\times180\degree/6\right)}$, respectively. Thus, the `timestamp' feature is replaced by 8 new, more informative features.

%\fi

%\emph{describe missing values; plot of number of samples vs number of missing values}
%\emph{structured data}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
%\subsection{Data Imputation}\label{sec:dataImputation}

%\tcr{(SCD: Should this perhaps go into the section on data?)}

%As we note in \S\ref{sec:data}, our dataset of 180,000 samples contains () samples with one or more missing values. This is not a concern when dealing with tree-based models, as they are natively able to handle splits with missing observations. Hence, we do not find it necessary to implement any kind of data imputation. However, for sake of completeness, we compare the predictions with and without implementing a K-Nearest Neighbors based imputation scheme \yst{If this is not necessary, I would omit. To explain K-nearst neighbours, you first need to define a metric, and how you define the distance if both data has missing values. All these are unclear to me.} \seb{don't we need the data-imputation from the NN, or SG is masking the missing values?} from Pandas\footnote{(insert hyperlink)}. As we show in Figure (), .....

%\tcr{SCD: Note the two sources of data imputation need to be combined into one}
%\fi

%\input{data_imputation}
%Additional Features

%\input{eda}

%\input{instruments}

==> Old_Files/introduction.tex <==
\section{Introduction}\label{sec:introduction}

%Image quality, usually defined by the full width at half maximum (FWHM) of the point spread function (PSF) of a point-like object (e.g. a star) by an imaging camera on a telescope, is the single most important metric of efficiency in astronomical observations, whether in pure imaging or in spectroscopic mode. 

%\yst{I suspect this can be "dumbed" down a little. maybe just emphasize how much PSF scale as observation time and hence \$\$?}Indeed, the variance of the flux of a star, estimated either via a maximum likelihood technique or in a circular aperture, is roughly proportional to the PSF area, which scales as the square of the FWHM \citep{Portillo2020}, while at the same time it is inversely proportional to the observation time (at least in the regime where it is dominated by photon noise). It is therefore of prime importance to reduce, as much as one can, the FWHM (a.k.a. "seeing" in astronomy) in order to improve telescope efficiency. 

%The image quality is directly related to the presence of turbulence in the different atmospheric layers above the telescope \citep[free atmosphere, boundary layer, surface layer, see ][]{Racine2005}, and therefore the properties of the observation site are of prime importance for the success of the telescope operations. Situated on top of the excellent site of Maunakea on the Big Island of Hawaii \citep{racine1993}, the image quality of the Canada-France-Hawaii Telescope (CFHT) was steadily improved since its first light, but never quite reached the quality expected from the site itself due to the presence of turbulence within its own enclosure that degrades further the image quality, due in part to a poor ventilation of the telescope dome \citep{racine1991mirror,salmon2009cfht,Pfrommer_2015}. This led to a sophisticated modelling of the impact of creating dome vents on the image quality, using both CFD and water tunnel tests \citep{Baril2012} \yst{this sentence seems a bit too detailed?}. These vents have since been opened \citep{bauman2014dome} and led to a significant reduction of the turbulence inside the dome and therefore an improved image quality.

%However, if the telescope image quality on the best nights becomes close to the limits of the site itself, there remains a significant fraction of observing nights where the telescope image quality is still far from the site's intrinsic limits. To improve further the image quality, two different approaches are ongoing: the first one consists of measuring the turbulence in situ at different locations within the dome using portable interferometers \citep{Lai20} \yst{slightly confused here, how does measuring the turbulence alone helps to reduce it?}, the second, which we describe in this paper, is purely data driven. 

% tentative of dumbed down intro below.
%\seb{The scientific productivity of the Canada France Hawaii Telescope (CFHT) can be explained greatly by the exceptional image quality at the summit of Maunakea on the Big Island of Hawaii. A standard definition of image quality, the Full Width at Half Max (FWHM) of the profile of a point source located above the atmosphere (a star), and measured on the science exposures. Effectively this is a metric which directly relates to the signal-to-noise of astronomical sources measurements.
%Since its first light in 1979, CFHT image quality has steadily improved by controlling the interior dome venting of the telescope, temperature control, and adapting the instruments hosted by the telescope. 
%Despite constant improvements, image quality at CFHT is only rarely reaching what the site theoretically could deliver. Science proposals often require the best reachable image qualities, and ideally forecasting image quality with sufficient time would help prioritise science proposals and instrument scheduling, ultimately using the observatory at its full potential.}

%\yst{I feel strongly this paragraph, at least part of it, should be the the first paragraph of the paper. It will set the tone right away. } 

In this paper we describe initial steps towards the first-ever machine-learning driven approach to real-time scheduling of astronomical observations at the Canada-France-Hawaii Telescope (CFHT). CFHT, sited on the summit of the 4,200m volcano of Maunakea on the island of Hawai'i, is one of the most productive ground-based observatories ~\cite{crabtree:2019}. The CFHT saw its first light in 1979 and has  amassed decades-worth of observation data. 
%Each data point includes the scientific image and hundreds of ancillary environmental and observatory dome operating parameters.

In this contribution, we present results on an interpretable deep neural network that outputs a predicted measure of the quality of an intended scientific exposure as a function of 
ancillary environmental and observatory dome operating parameters.
%environmental conditions (including temperature, pressure, and wind speeds measurements), various controllable dome parameters (dome vent, windscreen, and cooling settings), and dome ``pointing'', i.e., which astronomical object is to be observed.  
In the longer term, our goal is to use such predictors to schedule the sequence of observations and to control the dome to maximize image quality.  
Improved condition-dependent scheduling is key for at least two reasons.  First, the available ``observing'' time at CFHT each year is oversubscribed with science proposals by about $3 \times$.  Improving the efficiency and quality of telescope operation allows more valuable science targets to be observed in a given period. Secondly, the operation of the telescope is staggeringly expensive. For a 4m-class telescope like CFHT, it costs about USD \tcr{xx} per night to operate. And it is estimated that the next generation of 30m telescopes, such as GMT, TMT and ELT \tcr{[ref]}, will cost USD 100,000\tcr{(?)} per night (or USD \tcr{xx} per second) to operate. Due to these immense operating costs, 
%Second, while the data with which we work herein comes from the CFHT wide field optical imager ``Megaprime'', which can only be aimed at a single astronomical object in each exposure, the next generation instrument (the Maunakea Spectroscopic Explorer) will be able to be aimed at over \tcr{1000} distinct astronomical objects in a single exposure.  
%Thus, to increase scientific productivity, 
automation of the scheduling process and optimization of image quality is crucial.  
%We take the first steps towards that goal in this paper.

%% THE FOLLOWING IS NICE TEXT FROM SIMON, CAN WE WORK IT IN?
%Science proposals often require the best reachable image qualities, and ideally forecasting image quality with sufficient time would help prioritise science proposals and instrument scheduling, ultimately using the observatory at its full potential.

%The output of the neural network 
To quantify the quality of an exposure, we present a probabilistic prediction of image quality (known as ``IQ''). 
%We use the standard definition of IQ, {\em full width at half max} (FWHM). 
The IQ
%FWHM 
measures the point-source blurring (i.e., of a star) and relates directly to the signal-to-noise ratio of most scientific feature measurements made on the exposure.  IQ degradation from the theoretical maximum results from turbulent flow in the atmosphere and from in-dome turbulence induced by the night-time cooling of the dome itself.  The summit of Maunakea is a prime location for siting ground-based observatories (the other is in Chile) as atmospheric turbulence is minimal due to the smooth flow of the prevailing trade winds and the height of the Maunakea summit.  Despite steady improvements in CFHT IQ since 1979 --  by (rather ad-hoc) controlling the interior dome venting of the telescope, temperature control, and adapting the instruments hosted by the telescope -- IQ only rarely reaches what the site can theoretically deliver. Predicting and  taking action to reduce dome-induced turbulence is our immediate goal.  

The contributions of this papers are as follows.  First, we demonstrate that the ancillary environmental and operating data are sufficient to predict IQ to reasonable accuracy 
%(reasonable to astronomers!).  
Second, by implementing an interpretable deep neural network model we identify which sensor measurements are most informative in prediction the 20-years worth of IQ measurements at our disposal. Finally, by  optimizing the vent configurations used with these historical data, our models predict a substantial improvement in IQ.
%
\tcr{(SCD:Can we keep the following in, would be nice if we can, do we have a percentage?  It's also in the abstract. we can substantially reduce the running cost by XX\%.}
%
Our successes here lay the foundation for developing automated control approaches to improve image quality and, eventually, to solve the scheduling problem. 




%The question we are addressing here is the following: are these ancillary data sufficient to explain the image quality observed by Megacam ? Could machine learning help forecasting the image quality from these ancillary data? And if so with what accuracy, and what are the most relevant features such an algorithms find? The answer to this last question is fundamental to search for technical solutions to further improve the telescope's image quality.

%\SEB{Here we describe how we implemented an interpretable deep neural network with probabilistic predictions of image quality, and show which sensor measurements were actually relevant in predicting almost 20 years of image quality measurements. }% if it is the first time is this done?

%The rest of the paper is structured as follows.  In Sec.~\ref{sec:data}, we describe the data set used to train our network, in Sec.~\ref{sec:methods} we describe the ML techniques that we use for supervised learning and feature ranking. Finally, we present illustrative results and interpretations in Sec.~\ref{sec:results}.


==> Old_Files/introduction_orig.tex <==
\section{Introduction}\label{sec:introduction}

%In this paper
We delineate here initial steps towards the first-ever %machine-learnin
ML-driven approach to real-time scheduling of astronomical observations at the scientifically productive Canada-France-Hawaii Telescope (CFHT).
%, is one of the most productive ground-based observatories %~\cite{crabtree:2019},
Situated on the summit of the 4,200 m volcano of Maunakea on the island of Hawai'i, CFHT has gathered decades-worth of high-quality observation data since its first light in 1979.

Specifically, we create a neural network that predicts a measure of the quality of an intended scientific exposure as a function of ancillary environmental and observatory dome operating parameters. In the longer term, our goal is to use such predictors to schedule the sequence of observations and to action dome controls to maximize image quality. Improved condition-dependent scheduling is key for at least two reasons. First, the available ``observing'' time at CFHT is oversubscribed with science proposals by about $3 \times$.  Improving the efficiency and quality of telescope operation will allow more prioritized science targets to be observed in a given period. Second, CFHT costs around USD $25,000$ per night to operate, a quarter of what next generation 30m-class telescopes will cost. Automation of the scheduling process based on scientific quality is therefore time-critical.

To quantify the quality of an exposure, we implement a probabilistic prediction of image quality (IQ). IQ measures the point-source blurring of a star, and relates directly to the signal-to-noise ratio of most scientific feature measurements made on the exposure.  IQ degradation from the theoretical maximum results from turbulent flow in the atmosphere and from turbulence in the dome of the observatory induced by the night-time cooling of the dome itself. The summit of Maunakea is a prime location for siting ground-based observatories as atmospheric turbulence is minimal due to the smooth flow of the prevailing trade winds and the height of the summit.  Despite steady improvements in CFHT IQ since 1979 -- for example by installing vents in the dome to replace hot air in the interior with cool mountain air %controlling the interior dome venting and temperature of the telescope or adapting the instruments hosted by the telescope
-- IQ only rarely reaches what the site can theoretically deliver. Predicting and taking action to reduce dome-induced turbulence is our immediate goal.  

The contributions of this papers are as follows.  First, with the help of an interpretable and probabilistic deep neural network, we demonstrate that the ancillary environmental and operating data are sufficient to predict IQ to reasonable accuracy. Second, we identify which sensor measurements are most informative in our predictions, using the 20-years worth of IQ measurements at our disposal. Finally, by optimizing the vent configurations used with these historical data, our models predict a substantial improvement in IQ.
\tcr{(SCD:Can we keep the following in, would be nice if we can, do we have a percentage?  It's also in the abstract. we can substantially reduce the running cost by XX\%.} Our successes here lay the foundation for developing automated control approaches to improve image quality and, eventually, to solve the scheduling problem. 


\begin{figure}
   \centering
   \includegraphics[width=0.8\linewidth]{Fig1.png}
   \caption{The layout of the Canadian-France-Hawaii Telescope. Annotated are the 12 dome vents. By optimizing these vent configurations, we demonstrate we can reduce the dome induced turbulence and consequently the telescope operation costs.}
\end{figure}


==> Old_Files/method.tex <==
\section{Method} \label{sec:methods}
%- NGBoost and feature ranking\\
%- DNN+MDN

%While DNNs allow extraction of significantly richer patterns between inputs and output(s), they have earned a reputation for being `black-boxes'--it can be difficult to explain the series of steps a neural network takes to find the relationships between the input features and the output(s) of interest. Traditionally, \emph{structured}, tabular data has been processed with tree-based ML models such as random forests \citep{randomforests} and extremely randomized trees \citep{extremelyrandomizedtrees}; since these are agglomerations of if-then-else statements, it makes it very easy to analyze the inter-relationships among the input features and their relationship with the outputs. This increased interpretability comes at the cost of a weakened ability for feature extraction -- a machine learning model can only work with the user-provided features, whereas a deep enough neural network, in theory, can construct arbitrary complex combinations of these features if such an exercise results in better prediction of the output variable(s) of interest.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\iffalse
%At the beginning of this work we were faced with an interesting choice--whether to use a tree-based machine learning model, or a deep neural network (DNN). While DNNs allow extraction of significantly richer patterns between inputs and output(s), they have earned a reputation for being `black-boxes'--it can be difficult to explain the series of steps a neural network takes to find the relationships between the input features and the output(s) of interest. This is where tree-based models shine--they are designed to be agglomeration of `if-then-else' statements, thus making it considerably easier to inspect the relationships both between the input features and the outputs, as well as among the features themselves. They pay a price for increased interpretability with decreased ability for feature extraction\footnote{That is, a machine learning model can only work with the user-provided features, whereas a deep enough neural network, in theory, can construct arbitrary complex combinations of these features if such an exercise results in better prediction of the output variable(s) of interest.}, and often times are not the tools of choice for \emph{unstructured data}--images, videos, text and audio.[\textbf{CITATION NEEDED}].

%This performance hierarchy, however, is reversed in the case of \emph{structured}, tabular\footnote{Tabular data is considered `structured' because typically a human decides to put the features (columns) and observations (rows) in a certain order, whereas images, audio and languages have a naturally occurring order and do not need to be `structured' by the user.} data. While deep learning models are more appropriate in fields such as image recognition, speech recognition and natural language processing, tree-based models more often than not outperform standard deep models on tabular-style datasets [\textbf{CITATION NEEDED}], where features are individually meaningful and lack strong multi-scale temporal or spatial structures; the state-of-the-art performance in problems with tabular heterogeneous data is often achieved by such as gradient boosted decision trees (GBDT) \citep{gradient_boosted_decision_trees_gbdt, xgboost, catboost}.

%This raises two questions: (i) \emph{why} does deep learning perform poorly on tabular data, and (ii) \emph{how} can we fix it? \seb{not exactly sure that DL can be said to perform poorly on tabular data anymore - as it is examplified here.} \yst{agreed. This is an unnecessary shot/comparison} The key to answering question (i) is to understand the ways in which tabular data are fundamentally different from unstructured data:
\begin{itemize}
%    \item They are heterogeneous--the features that go into a table often come from disparate sources, each with their own units. This is certainly true for the data that we use--as we explain in \S\ref{sec:data}, our features are a combination of environmental sensor measurements, dome meta-data, and instrumental image qualities. They have units as diverse as degree Celsius for temperatures, knots for wind-speed, and degrees for telescope azimuth.
%    \item They are sparse--unlike data from audio, video and language, there can be relatively little variation in the values of a column in a table. There are often NULL values where no data was collected, or was lost or corrupted in the collation process.
  %  \item They are categorical--tables often contain more categorical features, for example: is the wind speed $< 5$ knots, between $5$ and $10$ knots, between $10$ and $20$ knots, or $>20$ knots (\S\ref{sec:data_cleaning_feature_engineering}). These are discrete by nature, and are not dependent on the order or the numerical values of the features themselves (i.e., we do not care what the exact wind speed in knots is).
   % \item They are correlated--a minority of the columns in a table are often responsible for the majority of the predictive power. This is unlike the case for images, for instance, where in spite of local spatial correlations between pixels, it is difficult to claim that it is the top-left cluster of them that is most helpful in predicting whether an image contains a cat or a dog.
\end{itemize}

%These issues complicate analysis of tabular data with DNNs. These differences from unstructured data lead to a sparse and discontinous high-dimensional feature space, making it difficult to exploit for a typical DNN \textbf{citation}. On the other hand, tree-based models--decision trees \citep{decision_trees}, random forests \citep{randomforests}, and gradient boosted trees \citep{xgboost}--naturally profit from this landscape. They are by design able to select and combine features via a greedy heuristic, and thus whittle down the list of pertinent features to just the most predictive ones. They are also able to easily handle categorical features using any number of encoding schemes, the most commonly used one being one-hot encoding \textbf{insert citation}. The sparsity of features and the presence of NULL values is not of concern to them either, since they simply do not include feature cells containing such values in their splits.

%Before we answer question (ii) above, i.e., how do we fix the sub-par performance of DNNs on tabular data, we must answer another question. Given the ease of use and conventionally superior performance of tree-based models on tabular data, why consider DNNs at all?
\begin{itemize}
%    \item DNNs are powerful feature pre-processors. Using back-propagation, they learn a fine-tuned hierarchical representation of data by mapping input features to the output label(s). This allows us to shift our focus from feature engineering to fine-tuning the architecture, designing better loss functions, and generally experimenting with the mechanics of our neural network. This exact functionality allows us to get away with merely using the pairwise differences of the temperature values in \S\ref{sec:data_cleaning_feature_engineering} as additional, hand-crafted features.
%    \item There is empirical proof that DNNs result in improved performance with larger sized datasets \citep{airbnb}.
 %   \item Deep learning allows us to train systems end-to-end, which unlocks the possibility of using unlabelled samples to better predict the labelled ones (\emph{semi-supervised learning}, \S\ref{sec:DL_SSL}).
  %  \item It is easier to use DNNs in an online-mode, with data points `streaming in' rather than arriving in batches. This is because tree-based models need access to all the data to determine best split points, and hence need to be trained every time a new observation comes in. While this work does not use streaming data, in preparation for our future work on real-time predictions we believe it best to move to a neural network from the get-go.
    
%    \seb{another item: tree based often do not generalize well, i.e. extrapolate, even for simple model such as linear}.
\end{itemize}
%\input{tabnet}

%\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The ideal model of choice would thus enable us to leverage the advantages of both neural networks and tree-based models -- richer feature extraction from the former, and interpretability for end-user from the latter. Fortunately, the past few years have seen extensive research into designing exactly such DNNs, specialized to beat their ML-based cousins on structured data. While some mimic decision tree ensembles \citep{node}, others focus on developing novel architectures using attention \citep{attention_is_all_you_need} suitable for handling tabular data \citep{selfattention_feature_importance, tabnet}. 

We now describe the deep neural network we built which excels in feature extraction, and provides some significant interpretability for the end-user.  We implemented a modified version of the `TabNet' architecture \citep{tabnet}.
%, with several improvements. 
TabNet uses a sparse, learnable mask on the input features.
%--a kind of soft feature selection that favors the selection of just features that are important for the sample under consideration. %It uses a special type of non-linearity called `sparsemax' \textbf{sparsemax citation}, along with an \emph{attention mechanism} \citep{attention_is_all_you_need} called `self-attention' to zero out the contributions of non-relevant features in through a sequence of several steps.
%TabNet is also able to naturally normalize features of varying ranges, and thus does not require feature pre-processing. For a more detailed description and a visual overview of their network, we refer the readers to \S$2$ and Figure 4, respectively, of \cite{tabnet}. While TabNet has feature interpretability built-in, it can only output the magnitude of the impact of a feature on the output, and not its direction. In other words, it cannot discriminate a feature positively impacting the MPIQ from a feature negatively impacting it, except in magnitude of their effects. For this reason, we do not use this functionality, and instead utilize the \textrm{pathexplain} %\footnote{\url{https://github.com/suinleelab/path_explain}}
This choice is partly prompted by the built-in interpretability of TabNet, which allows for the extraction of feature importance
\citep{explaining_explanations_hessians}. \yst{Since we are probably not going to show the feature ranking, we can add a paragraph explaining the feature ranking seems to be physically sensible in an additional paragraph.}
\seb{we need a justification to show what the interpretability of TabNet brings to this project. The SHAP values could also be computed with a simple MLP.}
%package to obtain feature importance.
%Based on integrated Hessians, this allows us to convert a `black-box' DNN into a `glass-box'. 
%It is able to provide both \emph{feature attributions}--'how important is feature A relative to all other features in explaining the MPIQ?', and \emph{feature interactions}--'how does feature A's impact on MPIQ change in presence of feature B?'. We are thus able to analyze the impact of our features from multiple points of view.

Unlike in the original paper, in this study, we wrap TabNet as part of a mixture density network [REF] to provide probabilistic output of the seeing. \yst{some brief introduction about MDN- at most three sentences}. In particular, the estimate the aleatoric and epistemic uncertainties of our inference via the MDN output. \yst{define how the MDN output is defined as the aleatoric and epistemic}.

The training is done via a 8-2 split of the training data. \yst{explain in at most in one more sentence about the validation split.}
%We divide the CFHT-dataset into two parts: a training set $D_{\rm train}$ containing 80\% of samples, and a test set $D_{\rm test}$ containing the rest. We do this in a stratified way, %\footnote{We plot a histogram of the MPIQ values, and starting from the lowest value, put each point into one of the ten buckets generated for a 80-20 split.},
%o ensure that each set has a similar distribution of MPIQ values as the original dataset. We then re-divide the training set--again in a stratified way--into two sets using again a 90-10 split, with the first set $D_{\rm train-train}$ used for training our model, and the second, validation set $D_{\rm train-val}$ to choose the best hyperparameters for the model. We do this in a rotating fashion so after 10 rounds, every sample has been in a unique validation set. 
We optimize the training via AutoML framework,
%utilize an Automatic Machine Learning (AutoML) \citep{automl} framework, 
TPOT \citep{tpot}, for finding the best hyperparameters.%, that result in the lowest loss function. 
%For this, we use the log-cosine-hyperbolic [] function, which is less impacted by the tails of the MPIQ distribution than the more commonly used mean-squared-error (MSE) and mean-absolute-error (MAE) loss functions. Once we have final predictions (consisting of a mean $\mu$ and a standard-deviation $\sigma$ from the final `super-model' (with NGBoost at its head) for all samples (by training on a training set, predicting on the validation set, and repeating this 10 times), we \textbf{calibrate the predicted probabilities}. This is a post-processing step that corrects for the fact that the probabilities/uncertainties predicted by a model might not necessarily reflect the true underlying probabilities of the quantity of interest (in our case, MPIQ). 
%We use the best model output by TPOT, train it on the full training set $D_{\rm train}$, and predict the MPIQ $\mu$ and $\sigma$ for the test set $D_{\rm test}$. We then utilize the simple yet effective calibration method CRUDE \citep{crude_probability_calibration} to modify the predictions on the test set based on the predictions on the 10 validation sets. In Figure (), we show compare calibration curves with and without probability calibration correction. %\yst{I don't think we have talked about how we renormalized training set.}

%Secondly, we upgrade TabNet to output both upper and lower $1-\sigma$ quantiles instead of point predictions; this enables us to quantize the model's confidence in its output \citep{kendall2017uncertainties, choi2018uncertainty}. We do this by using 

%Thirdly, we divide \emph{predictive uncertainty} into two parts--\emph{aleatoric} and \emph{epistemic}  \cite{kendall2017uncertainties}. Aleatoric uncertainty captures the uncertainty in the data generating process--for example, measurement noise in filters, or the inherent randomness of a coin flipping experiment. It cannot be reduced by collecting more training data%\footnote{We know that a fair coin has a 0.5 probability of landing heads, yet we cannot assert with 100\% certainty the outcome of the next flip, no matter how many times we have already flipped the coin.} 
%; however, it can be reduced by collecting more informative features. On the other hand, epistemic uncertainty models the ignorance of the predictive model, and can indeed be explained away given an a sufficiently large training dataset. %\footnote{If we are given a biased coin where we do not know the probability $p$ of turning up heads, we can determine it to arbitrary precision by flipping the coin an arbitrarily large number of times and counting the number of times it turns up heads.}.
%Aleatoric uncertainty is thus sometimes referred to as \emph{irreducible} uncertainty, epistemic being its \emph{reducible} cousin. Aleatoric uncertainty covers first two of the four issues above, while epistemic uncertainty subsumes the last two. High aleatoric uncertainty can be indicative of noisy measurements or missing informative features, while high epistemic uncertainty could be a pointer to its status as an outlier.

%\begin{figure}{r}{0.5\textwidth}
%  \begin{center}
%    \includegraphics[width=0.48\textwidth]{cal_rebalanced_kanoa_20200905-175342.png}
%  \end{center}
%  \caption{\yst{We should not wrap figure. This really agitates reviewer. I would make the figure span a longer width even it break the 1-to-1 ratio.}}
%\end{figure}


\begin{figure}
 \centering
 \begin{subfigure}{0.5\textwidth}
   \centering
   \includegraphics[width=0.9\linewidth]{cal_rebalanced_kanoa_20200905-175342.png}
   \caption{Predicted vs.~true IQ}
 \end{subfigure}%
 \begin{subfigure}{0.5\textwidth}
   \centering
   \includegraphics[width=0.9\linewidth]{effect_ventconfigs.png}
   \caption{Predicted improved IQ vs.~nominal IQ}
 \end{subfigure}
\end{figure}

Finally, we further calibrate the probabilistic output our model
%post-process our model's predictions by calibrating the quantiles \citep{crude_probability_calibration}. 
In practice, most uncertainty estimates often fail to capture the underlying data distribution, and tend to underestimate the uncertainty \citep{lakshminarayanan_probability_calibration0, probability_calibration1, crude_probability_calibration}. The calibration is done via the CRUDE method
%We then utilize the simple yet effective calibration method CRUDE \citep{crude_probability_calibration} to modify the predictions on the test set based on the predictions on the 10 validation sets. 
\yst{explain in two sentences how CRUDE works.}%For example, a 95 \% confidence interval generally does not contain the true outcome 95\% of the time. When this happens, the model is said to be \emph{miscalibrated}. 
%This is caused by model overconfidence: just as a deterministic model is unable to determine its own ignorance \textbf{CITATION NEEDED}, a probabilistic model may not be powerful enough to map the right probability to its confidence interval. 
%Calibration is not directly measured by proper scoring rules like negative log likelihood \citep{measuring_calibration_in_deep_learning}. Since this is precisely the error which is the error metric we use (see \S\ref{sec:DL_MDN}), we need to correct the uncalibrated probabilities our model outputs.

%\textbf{\underline{metrics}}
%Here, we use the CRUDE method of \cite{crude_probability_calibration} to \emph{post-hoc} re-calibrate our model's \textbf{INSERT MODEL NAME HERE} predictions. This method ensures that not only are the post-processed predictions \emph{calibrated}, but that they are also \emph{sharp}. Ideally, each expected calibration percentile should match the fraction of values observed below the predictions of that percentile \citep{measuring_calibration_in_deep_learning}. Calibration is thus a joint property of the predicted and the ground truth values. Sharpness, on the other hand, refers to the concentration of the predictions--the more concentrated the predictive distributions are, the sharper the forecasts, and the sharper the better (provided it is not at the expense of calibration). \cite{crude_probability_calibration} show that CRUDE not only results in better calibrated predictions compared to previously proposed methods, but also sharper predictions.



\iffalse
\subsection{Mixture Density Network}\label{sec:DL_MDN}

Mixture density networks (MDNs) are built from two components: a neural network and a mixture model\footnote{First proposed in \cite{bishop_mdn}, they utilized a Gaussian mixture model (GMM), but can be easily generalized to work with an arbitrary distribution or even different types of distribution families.}. We begin by introducing the concept of a mixture model--a model of probability distributions built up from a weighted sum of more simple distributions. More concretely, we consider a one-dimensional distribution with $m$ mixture components. The probability density function (PDF) $p(x)$ is represented by the $m$ PDFs indexed by $j p_{j}(x),$ with weights $\Omega=\left\{\omega_{0}, \ldots, \omega_{m-1}\right\}$, where $\sum_{j=0}^{m-1} \omega_{j}=1$, by the following equation
\[
p(x)=\sum_{j=0}^{m-1} \omega_{j} p_{j}(x)
\]
Typically these probability distributions will be parameterised by a series of parameters that reflect the shape and location of the distribution $\Theta=\left\{\theta_{0}, \ldots, \theta_{m-1}\right\} .$ The full parameterised model may therefore be written as
\[
p(x \mid \Omega, \Theta)=\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x \mid \theta_{j}\right)
\]
As an example, each $p_{j}$ could be a normal distribution parameterised by a mean $\mu_{j}$ and a variance $\sigma_{j}$. The mixture model would then have the following form,
\[
p(x \mid \Omega, \Theta)=\sum_{j=0}^{m-1} \frac{\omega_{j}}{\sqrt{2 \pi \sigma_{j}^{2}}} \exp \left(\frac{-1}{2 \sigma_{j}^{2}}\left(x-\mu_{j}\right)^{2}\right)
\]
In general, these mixture distributions are multi-modal, including those in the form of Eq
$(4),$ and can be fitted directly to some data $\mathbf{x}=\left(x_{0}, \ldots, x_{n-1}\right) .$ Assuming independence, the corresponding likelihood is calculated as
\[
l(\mathbf{x} \mid \Omega, \Theta)=\prod_{i=0}^{n-1}\left[\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x_{i} \mid \theta_{j}\right)\right]
\]
Fitting can then typically proceed using expectation-maximisation [20] \yst{Is this correct? For our case, there are no classes, the training should only be a maximum likelihood. Am I missing something here? Or do you mean classical GMM here. I would shorten this.}. For our purposes, we have an individual-based model $M,$ with some input $\alpha,$ that produces stochastic realisations $y \sim M(\alpha) .$ We therefore wish to derive a relationship between the input parameters $\alpha,$ and the mixture density weights $\omega_{j}(\alpha)$ and density parameterisations $\theta_{j}(\alpha) .$ This could potentially be done with a separate regression for each of the density parameters and weights, although this would fail to capture the corresponding relationships that would exist between each parameter and weight. We can therefore model these using a neural network, which is able to provide flexible fitting for arbitrarily complex relationships by the universal approximation theorem
$[22] .$ An MDN is therefore defined as a mixture model, where the mixture components are modelled using a neural network. Fig 1 provides an overview of the MDN construction. The inputs of the model $\alpha$ are initially fed into the MDN (three such inputs in the example diagram). These are then passed through a number of hidden layers in the neural network, which provide a compact representation of the relationship between the inputs and the unnormalised inputs into the mixture model. These distribution parameters are then passed through a normalisation layer; the weights of the mixture are transformed such that they sum to one and the shape parameters are transformed so that they are positive. These parameters are used to construct the mixture model, where one can draw samples or calculate statistics, such as mean and variance, for a given input. For multiple outputs the final layer can be copied with independdent parameters for the number of outputs being considered \yst{Not sure I follow the last sentence here?}. Note that a number of aspects of the MDN need to be specified including the number of input parameters, the dimension of the output, the distributions used in the mixture density, and the number and size of the hidden layers.
The MDN can then be fit to the following objective loss function, which is equivalent to maximising the likelihood given in $\mathrm{Eq}(5)$
\[
f(\mathbf{x} \mid \Omega, \Theta)=-\sum_{i=0}^{n-1} \log \left(\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x_{i} \mid \theta_{j}\right)\right)
\]
Note that provided $p_{j}$ is differentiable with respect to $\theta_{j}$, this loss represents a differentiable function. Standard techniques based on stochastic gradient descent can then be applied in order to optimise the weights of the network with respect to this loss [23]

Mixture density networks (MDN) (Bishop, 1994) are a class of models obtained by combining a conventional neural network with a mixture density model.
We use a mixture of 20 normal distributions parameterized by a feedforward network. That is, the membership probabilities and per-component mean and standard deviation are given by the output of a feedforward network.


The standard normal--or Gaussian--distribution acts as the
foundation for countless modeling approaches in statistics
and machine learning. As opposed to a single Gaussian,
which is a very limited model, \emph{Gaussian mixture models} can represent or approximate almost any density
of interest while remaining intuitive and easy to handle. A Gaussian is characterized by two parameters--mean $\mu$ and standard deviation $\sigma$. We see from Figure () that our output label of interest, MPIQ, does not resemble a Gaussian

\yst{I think here you also need to explain how you define aleatoric and epistemic uncertainties from the MDN output. E.g, sigma of the mean, and mean of the sigma.}
\fi

\iffalse
\subsection{Probability Calibration}\label{sec:DL_probability_calibration}
Above, we describe the procedure for obtaining both aleatoric and epistemic errors from a deep neural network. However, not all errors are created equal--in practice, most uncertainty estimates often fail to capture the underlying data distribution \citep{lakshminarayanan_probability_calibration0, probability_calibration1, crude_probability_calibration}. For example, a 95 \% confidence interval generally does not contain the true outcome 95\% of the time (see Figure ()). When this happens, the model is said to be \emph{miscalibrated}. This is caused by model overconfidence: just as a deterministic model is unable to determine its own ignorance \textbf{CITATION NEEDED}, a probabilistic model may not be powerful enough to map the right probability to its confidence interval. Calibration is not directly measured by proper scoring rules like negative log likelihood \citep{measuring_calibration_in_deep_learning}. Since this is precisely the error which is the error metric we use (see \S\ref{sec:DL_MDN}), we need to correct the uncalibrated probabilities our model outputs.

Here, we use the CRUDE method of \cite{crude_probability_calibration} to \emph{post-hoc} re-calibrate our model's \textbf{INSERT MODEL NAME HERE} predictions. This method ensures that not only are the post-processed predictions \emph{calibrated}, but that they are also \emph{sharp}. Ideally, each expected calibration percentile should match the fraction of values observed below the predictions of that percentile \citep{measuring_calibration_in_deep_learning}. Calibration is thus a joint property of the predicted and the ground truth values. Sharpness, on the other hand, refers to the concentration of the predictions--the more concentrated the predictive distributions are, the sharper the forecasts, and the sharper the better (provided it is not at the expense of calibration). \cite{crude_probability_calibration} show that CRUDE not only results in better calibrated predictions compared to previously proposed methods, but also sharper predictions.


Finally, to measure the degree of calibration, we use two metrics (described in detail in \S\ref{sec:DL_metrics}): Average Coverage Error (ACE) and Prediction Interval Normalized Average Width (PINAW). To measure the sharpness of the predicted probability distributions, we utilize Interval Sharpness (IS). Finally, we use the Continuous Ranked Probability Score (CRPS) to simultaneously evaluate both the degree of calibration and sharpness. % cite \textbf{`CuttingEdge_Technologies_for_Renewable_Energy_Production_and_Storage chapter 4'}.


We divide the CFHT-dataset into two parts: a training set $D_{tr}$ containing 90\% of samples, and a test set $D_{tst}$ containing the rest. We do this in a stratified way\footnote{We plot a histogram of the MPIQ values, and starting from the lowest value, put each point into one of the ten buckets generated for a 90-10 split. \footnote{Is this not the same as saying we randomize, and "hold-out" 90-10 split for each training?}}, to ensure that each set has a similar distribution of MPIQ values as the original dataset. We then re-divide the training set--again in a stratified way--into two sets using again a 90-10 split, with the first set $T_{tr_tr}$ used for training our model, and the second, validation set $T_{tr_val}$ to choose the best hyperparameters for the model. We do this in a rotating fashion so after 10 rounds, every sample has been in a unique validation set. We utilize an Automatic Machine Learning (AutoML) \citep{automl} framework, TPOT \citep{tpot}, for finding the best hyperparameters, that result in the lowest loss function. For this, we use the log-cosine-hyperbolic [] function, which is less impacted by the tails of the MPIQ distribution than the more commonly used mean-squared-error (MSE) and mean-absolute-error (MAE) loss functions. Once we have final predictions (consisting of a mean $\mu$ and a standard-deviation $\sigma$ from the final `super-model' (with NGBoost at its head) \yst{explain how a tree based model generate probalistic output. This is not clear to me} for all samples (by training on a training set, predicting on the validation set, and repeating this 10 times), we \textbf{calibrate the predicted probabilities}. This is a post-processing step that corrects for the fact that the probabilities/uncertainties predicted by a model might not necessarily reflect the true underlying probabilities of the quantity of interest (in our case, MPIQ). We use the best model output by TPOT, train it on the full training set $T_{tr}$, and predict the MPIQ $\mu$ and $\sigma$ for the test set $T_{tst}$. We then utilize the simple yet effective calibration method CRUDE \citep{crude_probability_calibration} to modify the predictions on the test set based on the predictions on the 10 validation sets. In Figure (), we show compare calibration curves with and without probability calibration correction. \yst{I don't think we have talked about how we renormalized training set.}


\subsection{Performance Metrics}\label{sec:DL_metrics}
\textbf{\underline{Metrics for Deterministic Predictions}}

\yst{Since we end up doing probablistic networks, is this subsection still relevant?}

For determining the `goodness' of point/deterministic predictions, we adopt the following four performance criteria:
\begin{itemize}
    \item Root mean square error (RMSE):
    \begin{align}
        \mathrm{RMSE}=\sqrt{\frac{1}{n} \sum_{i=1}^{n}\left(\tilde{y}(i)-y(i)\right)^{2}},
    \end{align}
    \item Mean absolute error (MAE):
    \begin{align}
        \mathrm{MAE}=\frac{1}{n} \sum_{i=1}^{n}\left|\tilde{y}(i)-y(i)\right|,
    \end{align}
    \item Normalized mean absolute percentage error (NMAPE):
    \begin{align}
        \mathrm{NMAPE}=\frac{1}{n} \sum_{i=1}^{n} \frac{\left|\tilde{y}(i)-y(i)\right|}{\max _{i \in 1, \mathrm{n}]} y(i)} \times 100 \%,
    \end{align}
    \item Bias:
    \begin{align}
        \mathrm{Bias} = \sum_{i=1}^{n} \tilde{y}(i)-y(i),
    \end{align}
\end{itemize}
where $y(i)$ and $\tilde{y}(i)$ are the true and predicted values of the $i^{th}$ sample in the test set, while $n$ is the total number of samples in the test set. A perfect prediction would result in RMSE, MAE, NMAPE, and Bias of 0.

\textbf{\underline{Metrics for Probabilistic Predictions}}
%\yst{This seems unnecessarily complex. What advantage do they provide than just a simple likelihood.}--NLL doesn't optimize calibration.
Probabilistic predictions are assessed by constructing Confidence Intervals (CI) and using them in evaluation criteria. In this work, we adopt the following four:
\begin{itemize}
    \item Average Coverage Error. ACE is an indicator to appraise the reliability of prediction interval, which has the following equation:
    \begin{align}
        \mathrm{ACE}_{\alpha}=\frac{1}{n} \sum_{i=1}^{n} c_{i} \times 100 \%-100 \cdot(1-\alpha) \%,
    \end{align}
    where $c_i$ is the indicative function of coverage and its calculation equation is as:
    \begin{align}
        c_{i}=\left\{\begin{array}{l}
1, y(i) \in\left[l_{\alpha}(i), u_{\alpha}(i)\right] \\
0, y(i) \notin\left[l_{\alpha}(i), u_{\alpha}(i)\right]
\end{array}\right.
    \end{align}
    ACE is effectively the ratio of target values falling within the confidence interval to the total number of predicted samples.
    \yst{What interval(s) CRUDE adopt for the calibration?}
    \item Prediction Interval Normalized Average Width (PINAW):
    \begin{align}
        \mathrm{PINAW} = \frac{\sum_{i=1}^n U_i - L_i}{nr},
    \end{align}
    where $r = y_{max} - y_{min}$. PINAW is the mean of PI widths normalized by the range of testing targets. \yst{I think this needs to be elaborated. Like what is $U_i$. I am not sure I follow this part.}
    \item Interval Sharpness (IS):
    \begin{align}
        \mathrm{IS}_{\alpha}=\frac{1}{n} \sum_{t=1}^{n}\left\{\begin{array}{ll}
-2 \alpha\Delta_{\alpha}(i)-4\left[l_{\alpha}(t)-y(t)\right], & y(t)<l_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i)-4\left[y(t)-u_{\alpha}(t)\right], & y(t)>u_{\alpha}(t) \\
-2 \alpha\Delta_{\alpha}(i), & \mathrm{otherwise}\end{array}\right.
    \end{align}
    where $\Delta_{\alpha}(i) = u_{\alpha}(i)-l_{\alpha}(i)$. \yst{same for here..}
    \item Continuous Ranked Probability Score (CRPS):
    \begin{align}
        \mathrm{CRPS}=\int_{-\infty}^{\infty}(F(y)-\mathbb{1}(y-x))^{2} d y,
    \end{align}
    where $F$ is the cumulative distribution function (CDF) associated with the probabilistic forecast, and $\mathbb{1}$ is the Heaviside step function.
\end{itemize}
From the equation of ACE, a value close to zero denotes the high reliability of prediction interval. As an infinitely wide prediction interval is meaningless, IS is another indicator contrary to the coverage rate of interval, which measures the accuracy of probabilistic forecasting. $\mathrm{IS}_{\alpha}$ is always $<0$; a great prediction interval obtains high reliability with a narrow width, which has a small absolute value of IS. PINAW is the mean of PI \yst{predictive interval?} widths normalized by the range of testing targets. Our goal is to ensure that PI is not too wide, since that would make it useless as a metric. The CRPS is a measure of the integrated squared difference between the cumulative distribution function of the forecasts and the corresponding cumulative distribution function of the
observations. It CRPS generalizes the mean absolute error (MAE), and reduces to it if the forecast is deterministic. It simultaneously considers the reliability and sharpness, and is a commonly used metric to evaluated the performance of the predicted conditional PDF. Note that CRPS is the only metric that uses the raw predicted PDF, and not the predicted intervals obtained by using Equation (). \yst{The overall intuition is straightforward, but I think this section requires some serious rewriting such that it is clear as a standalone piece.} \yst{If IS and CRPS are not used in CRUDE, but rather we are only using them as a post-validation, I would recommend removing them. I guess it is more visual just to show the plot.}
\textbf{MAKE SURE THIS ABOVE PARA ISN'T PLAGIARIZED; I HAVE A VAGUE RECOLLECTION OF COPYING SOME BITS FROM SOMEWHERE WITH THE INTENTION OF LATER MODIFYING THEM.}
\fi


\iffalse
\input{feature_ranking}

\input{data_imputation}

\input{errors}

\input{mdn}

\input{calibration}

\input{metrics}

\input{ssl}

%\input{feature_imp}

\input{putting_it_all_together}
\fi
%%%%%%%%%%%%
%\subsection{Semi-supervised}
%\label{sec:semiSupervised}

==> Old_Files/method_old.tex <==
\section{Method} \label{sec:methods}

% \begin{figure}
% \centering
%  \begin{subfigure}[b]{0.49\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{cfht_network.png}
%      \caption{$y=x$}
%      \label{fig:nn_architecture}
%  \end{subfigure}
%  \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{attributions_small.pdf}
%      \caption{$y=3sinx$}
%  \label{fig:feature_importance}
% \end{subfigure}
% \end{figure}

We implement a feed-forward network with ResNet style architecture and generalized linear unit (GLU) activation function in TensorFlow \cite{tensorflow2015-whitepaper}, as shown in Figure \ref{fig:nn_architecture}. %, drawing inspiration from the `TabNet' architecture \citep{tabnet}. While TabNet is also able to naturally normalize features of varying ranges, and thus does not require feature pre-processing. While the latter was designed in the style of a tree to iteratively select feature most impactful on predicting the output of interest, it can only output the magnitude of such impact, and not its direction. In other words, it cannot discriminate a feature positively impacting the MPIQ from a feature negatively impacting it, except in magnitude of their effects.
We utilize the \textrm{pathexplain} python package \footnote{\url{https://github.com/suinleelab/path_explain}} to obtain global feature importances. This enables us to answer two questions simultaneously---how important is a particular feature relative to all other features in explaining the image quality, and how does the IQ change with change in a given feature's values. We wrap this MLP as part of a mixture density network (MDN) \cite{bishop_mdn} to provide probabilistic output of the image quality. An MDN is a model of probability distributions comprising a weighted sum of simpler distributions---where the mixture components are modelled using a neural network. These mixture distributions are multi-modal, and are fitted directly to the input features $\mathbf{x}=\left(x_{0}, \ldots, x_{n-1}\right) .$ If we consider a one-dimensional distribution with $m$ mixture components, the probability density function (PDF) of the mixture, $p(x)$, is represented by the $m$ PDFs indexed by $j p_{j}(x),$ with weights $\Omega=\left\{\omega_{0}, \ldots, \omega_{m-1}\right\}$ -- where $\sum_{j=0}^{m-1} \omega_{j}=1$ -- by $p(x)=\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x\mid \theta_{j}\right)$; the $\theta$s contain information about the shape and location of the underlying distribution. Here we choose $m=50$, and $p_{j}(x)$s as Beta distributions, and fit our MDN to the negative-log-likelihood (NLL) loss function, given by $f(\mathbf{x} \mid \Omega, \Theta)=-\sum_{i=0}^{n-1} \log \left(\sum_{j=0}^{m-1} \omega_{j} p_{j}\left(x_{i} \mid \theta_{j}\right)\right)$.% This is equivalent to maximizing the likelihood.

Thus for each sample $x_i$, we obtain $m \times 3$ parameters: each of the $m$ mixture component comprises has 2 parameters for the Beta distribution -- which are converted to mean and standard deviation using \textrm{TensorFlow} primitives -- and 1 parameter  $\omega_i$ denoting its contribution to the MDN. Using these, we obtain three statistics for each sample: (i) \emph{mean}, $\mu = \left(\sum_{j=0}^{m-1} \omega_{j} \mu_{j}\right)$, (ii) \emph{aleatoric uncertainty}, $\sigma_a^2 =  \sum_{j=0}^{m-1} \omega_{j} \sigma_{j}^{2}$, and (iii) \emph{epistemic uncertainty}, $\sigma_{e}^2 = \sum_{j=0}^{m-1} \omega_{j} \mu_{j}^{2} - \mu^{2}$. Aleatoric uncertainty, also known as \emph{irreduceable uncertainty}, arises from inherent stochasticity in the input. For example, measurement noise, and missing informative features. It cannot be reduced by collecting more samples. On the other hand, epistemic or \emph{reducible uncertainty} quantifies the model's uncertainty in parts of the parameter space sparsely populated by the training samples. It can be reduced by collecting more and diverse samples. The total uncertainty is derived by adding these in quadrature.


\iffalse
TabNet uses a sparse, learnable mask on the input features. This choice is partly prompted by the built-in interpretability of TabNet, which allows for the extraction of feature importance \citep{explaining_explanations_hessians}. TabNet uses a sparse, learnable mask on the input features.
This choice is partly prompted by the built-in interpretability of TabNet, which allows for the extraction of feature importance
\citep{explaining_explanations_hessians}. \yst{Since we are probably not going to show the feature ranking, we can add a paragraph explaining the feature ranking seems to be physically sensible in an additional paragraph.}
\seb{we need a justification to show what the interpretability of TabNet brings to this project. The SHAP values could also be computed with a simple MLP.}
\fi

%\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{center}
%    \includegraphics[width=0.48\textwidth]{Fig2.png}
% \end{center}
% \caption{The predictions of seeing via deep learning. We demonstrate that the telescope "seeing" (or image quality) can be predicted via both the configurable telescope parameters (e.g. vent configuration) and other environment conditions (e.g., wind, pressure).}
%\end{wrapfigure}

% \begin{wrapfig}
%     \centering
%     \includegraphics[width=0.5\textwidth]
%     \caption{$y=x$}
%     \label{fig:y equals x}
% \end{wrapfig}

These derived uncertainties are then post-processed to improve \emph{calibration}. This is because in practice, most uncertainty estimates often fail to capture the underlying data distribution \citep{lakshminarayanan_probability_calibration0, probability_calibration1, crude_probability_calibration}. For example, a $1-\sigma$ confidence interval generally does not contain the true outcome 68\% of the time. When this happens, the model is said to be \emph{miscalibrated}. This is caused by model overconfidence: just as a deterministic model is unable to determine its own ignorance, a probabilistic model may not be powerful enough to map the right probability to its confidence interval. %Calibration is not directly measured by proper scoring rules like NLL \citep{measuring_calibration_in_deep_learning} -- hence the need to to correct the uncalibrated probabilities from our model.
We use the CRUDE method of \cite{crude_probability_calibration} to \emph{post-hoc} re-calibrate our model's predictions. This method ensures that not only are the post-processed predictions \emph{calibrated}, but that they are also \emph{sharp}. Sharpness refers to the concentration of the predictions---the more peaked (i.e. sharper) the predictions are, the better, provided it is not at the expense of calibration. \cite{crude_probability_calibration} show that CRUDE not only results in better calibrated predictions compared to previously proposed methods, but also sharper predictions.

Finally, we use two sets of metrics to quantify our model's predictions. The sample means $\mu$s are used to calculate the root mean squared error (RMSE), the mean absolute error (MAE), and the bias error (BE) -- for all three, the smaller the better. The uncertainties are measured by the percentage of true values within $1-\sigma$ confidence interval (expected calibration error (ECE) + 0.6827), and interval sharpness (IS). For the former, the ideal value is 0.6827, while the latter should ideally be 1. We split the total input data into training and test sets via an 9-1 split. The training data is again divided into training and validation subsets via cross-validation with a 9-1 split. The model predictions on the validation splits are concatenated and used to calibrate the predictions on the held-out test set.

%\begin{figure}
%\centering
% \begin{subfigure}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{means_jointplot.png}
%     \caption{$y=x$}
%     \label{fig:y equals x}
% \end{subfigure}
% \hfill
%     \begin{subfigure}[b]{0.49\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{errors.pdf}
%     \caption{$y=3sinx$}
% \label{fig:three sin x}
%\end{subfigure}
%\end{figure}


\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{Fig3.png}
    \caption{Optimizing the vent configuration can dramatically improve the image quality of the telescope. The left panel shows the nominal vent configurations, and the middle the predicted optimal vent configuration that leads to the improvement as shown in the right panel.}
\end{figure}

==> Old_Files/results.tex <==
\section{Results}\label{sec:results}

\begin{wrapfigure}{L}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{attributions_temp.png}
  \end{center}
  \caption{Birds}
\end{wrapfigure}

asdfasdfasd
asdfasdfasdfa
fasdfasdfasdf
asdfasdfadsf
asdfasdfasdf
asdfasdfasdf

\iffalse

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{barplot_IQ.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{attributions_temp.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{cal_rebalanced_kanoa_20200905-175342.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

\fi

